Enhancing Instruction Prefetching via Cache and TLB Management

Modern server workloads exhibit massive instruction footprints that heavily pressure the processor front-end, making L1 instruction (L1I) prefetching critical for sustaining performance. However, this paper shows that current L1I prefetchers fail to reach their full potential due to two key limitations. First, L1I prefetches crossing page boundaries require address translation before issuance, and translation latency reduces prefetch timeliness. Second, the reuse behavior of code lines fetched by L1I prefetches is highly heterogeneous: while some lines are reused many times, others are dead-on-arrival. This paper introduces Instruction Prefetch-Centric Cache and TLB Management (IP-CaT), the first microarchitectural framework jointly optimizing TLB and cache management for L1I prefetching. IP-CaT consists of two components: (i) the translation Prefetch Buffer (tPB), a small structure colocated with the second-level TLB (sTLB) that stores page table entries fetched by page-crossing L1I prefetches, reducing translation overheads; and (ii) the Trimodal Instruction Prefetch Replacement Policy (TIPRP), a decision-tree-based L2 cache replacement policy specialized for lines fetched by L1I prefetches. We evaluate IP-CaT with three state-of-the-art L1I prefetchers: EPI, FNL+MMA, and Barca. Across 105 contemporary server workloads, IP-CaT consistently improves performance. For example, IP-CaT+EPI achieves an 8.7% geomean speedup over EPI alone. We further show that IP-CaT outperforms state-of-the-art instruction TLB prefetching, advanced TLB replacement (CHiRP), and state-of-the-art code-aware, prefetch-aware, and general-purpose cache replacement policies, including Emissary, SHiP++, and Mockingjay.

==> 09_artifact_evaluation.tex <==
\section{Artifact Appendix}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}

{\em Obligatory. Summarize your artifacts (including algorithms, models, data sets, software and hardware) 
and how they help to reproduce the key results from your paper.}

\subsection{Artifact check-list (meta-information)}

{\em Obligatory. Use just a few informal keywords in all fields applicable to your artifacts
and remove the rest. This information is needed to find appropriate reviewers and gradually 
unify artifact meta information in Digital Libraries.}

{\small
\begin{itemize}
  \item {\bf Algorithm: }
  \item {\bf Program: }
  \item {\bf Compilation: }
  \item {\bf Transformations: }
  \item {\bf Binary: }
  \item {\bf Model: }
  \item {\bf Data set: }
  \item {\bf Run-time environment: }
  \item {\bf Hardware: }
  \item {\bf Run-time state: }
  \item {\bf Execution: }
  \item {\bf Metrics: }
  \item {\bf Output: }
  \item {\bf Experiments: }
  \item {\bf How much disk space required (approximately)?: }
  \item {\bf How much time is needed to prepare workflow (approximately)?: }
  \item {\bf How much time is needed to complete experiments (approximately)?: }
  \item {\bf Publicly available?: }
  \item {\bf Code licenses (if publicly available)?: }
  \item {\bf Data licenses (if publicly available)?: }
  \item {\bf Workflow automation framework used?: }
  \item {\bf Archived (provide DOI)?: }
\end{itemize}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}

\subsubsection{How to access}

{\em Obligatory}

\subsubsection{Hardware dependencies}

\subsubsection{Software dependencies}

\subsubsection{Data sets}

\subsubsection{Models}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Installation}

{\em Obligatory}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment workflow}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation and expected results}

{\em Obligatory}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment customization}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Notes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Methodology}

Submission, reviewing and badging methodology:

\begin{itemize}
  \item \url{https://www.acm.org/publications/policies/artifact-review-and-badging-current}
  \item \url{https://cTuning.org/ae}
\end{itemize}
